Deformable Part Models are Convolutional Neural Networks

Deformable part models (DPMs) and convolutional neural networks (CNNs) are two widely used tools for visual recognition. They are typically viewed as distinct approaches: DPMs are graphical models (Markov random fields), while CNNs are "black-box" non-linear classifiers. In this paper, we show that a DPM can be formulated as a CNN, thus providing a novel synthesis of the two ideas. Our construction involves unrolling the DPM inference algorithm and mapping each step to an equivalent (and at times novel) CNN layer. From this perspective, it becomes natural to replace the standard image features used in DPM with a learned feature extractor. We call the resulting model DeepPyramid DPM and experimentally validate it on PASCAL VOC. DeepPyramid DPM significantly outperforms DPMs based on histograms of oriented gradients features (HOG) and slightly outperforms a comparable version of the recently introduced R-CNN detection system, while running an order of magnitude faster.

==> related.tex <==
\section{Related work}

Over the last decade, multi-class object recognition has been benchmarked and analyzed with dataset challenges, such as PASCAL VOC \cite{PASCAL-ijcv} and the ImageNet LSVRC \cite{ILSVRC12}.
In the early days of the PASCAL detection challenge, the Dalal-Triggs HOG+SVM model \cite{Dalal05} was one of the most accurate detection methods.
The Dalal-Triggs model consists of a single-template sliding-window SVM detector, discriminately trained on images in the histogram of orientated gradients (HOG) feature space.
Building on the success of HOG+SVM, Felzenszwalb \etal \cite{lsvm-pami} introduced deformable parts models, which can be thought of as a substantial evolution of the Dalal-Triggs model, providing a large boost in detection accuracy.
Unlike Dalal-Triggs, DPMs use multiple templates and parts to enhance the model's ability to detect and localize objects.
Since part locations are not necessarily provided in training datasets, DPMs have the ability to learn latent parts with a Latent SVM.
DPMs traditionally operate in the HOG feature space, but DPMs have been shown to work in feature spaces besides HOG.
For example, Ren and Ramanan improve DPM accuracy by using histograms of sparse codes (HSC) \cite{HSC}.
DPM can be seen as an innovative combination of earlier work on pictorial structures \cite{Felzenszwalb05,Fischler73} together with Dalal and Triggs' HOG+SVM and weakly-supervised learning algorithms.
One goal of this paper is to continue this evolution by re-visiting DPM in light of recent advances in feature learning \cite{decafICML,girshick2014rcnn,krizhevsky2012imagenet}.
%Later in this paper, we show that DPMs can be described as an instantiation of convolutional neural networks.

Neural networks have been successfully applied to a number of object recognition problems such as digit recognition \cite{lecun-89e} and face detection \cite{rowley1998neural}.
Recently, deep convolutional neural networks by Krizhevsky \etal \cite{krizhevsky2012imagenet} and others have offered substantial accuracy improvements for image classification.
Inspired by these improvements, a number of similar neural network architectures have arisen to perform object detection in addition to classification.
For example, OverFeat \cite{overfeat} performs coarse sliding-window detection on CNN feature pyramids.
At each rough location, OverFeat uses a regressor to predict the location of a nearby object.
A recent CNN-based object detector called DetectorNet \cite{DetectorNet} also performs object detection with a multi-scale CNN pyramid, somewhat similarily to OverFeat.
DetectorNet begins by training a CNN on an object detection dataset like PASCAL, and then does an additional training step that focuses on improving the CNN's object localization.
Currently, the most accurate object detection method for both ImageNet detection as well as PASCAL is Regions with Convolutional Neural Network Features (R-CNN) \cite{girshick2014rcnn}.
Unlike DetectorNet and OverFeat, R-CNN does not perform sliding-window detection; instead R-CNN begins by extracting a set of region proposals \cite{UijlingsIJCV2013} and classifies them with a linear SVM applied to CNN features.
In contrast to previous work on sliding-window detection with CNNs, we aim specifically to understand the relationship between DPMs and CNNs and to understand if the modeling techniques used in DPM are applicable to CNN features.
Given the pervasive use of DPM in the computer vision community, we believe that our findings will have broad impact.

\todo{could also mention: Farabet (vis-a-vis cnn feat pyramids), boureau's work on max pooling}

